Privacy-Preserving XGBoost Inference

Although machine learning (ML) is widely used for predictive tasks, there are important scenarios in which ML cannot be used or at least cannot achieve its full potential. A major barrier to adoption is the sensitive nature of predictive queries. Individual users may lack sufficiently rich datasets to train accurate models locally but also be unwilling to send sensitive queries to commercial services that vend such models. One central goal of privacy-preserving machine learning (PPML) is to enable users to submit encrypted queries to a remote ML service, receive encrypted results, and decrypt them locally. We aim at developing practical solutions for real-world privacy-preserving ML inference problems. In this paper, we propose a privacy-preserving XGBoost prediction algorithm, which we have implemented and evaluated empirically on AWS SageMaker. Experimental results indicate that our algorithm is efficient enough to be used in real ML production environments.

==> ppxgboost.tex <==

\pprotocol{s}{$\ppxgboost$: A privacy-preserving $\xgboost$ inference
algorithm}{fig:algo}{htbp}
{\scriptsize
\textbf{$\setup$ Phase:}\\
\textbf{Input}: Plaintext model $\Omega$; Security parameter $k$; Model hyper-parameter $\alpha$.

Proxy computes: 
    
    \begin{itemize}[noitemsep,nolistsep,label={-}]
        \item $K_1 \larr \OPE.\Gen(1^k)$;
        \item $(\pk, \sk) \larr \she.\Gen(1^k)$;
        \item Choose $f$ uniformly at random from ${\mathcal F}_k$ in the PRF family;
        \item Choose $K_2$ uniformly at random from $\{0,1\}^k$;
        \item For each CART $T_i\in \Omega$, construct $T_i^\prime$ in $\encml$ as follows:
        \begin{itemize}[noitemsep,nolistsep]
         \item $T_i^\prime$ is structurally isomorphic to $T_i$.  
              Let $\phi: T_i \rarr T_i^\prime$ be an isomorphism;
         \item For each internal node $x$ with value $\vect{v}$ in $T_i$, 
              assign the value $\OPE.\Enc(K_1, \vect{v})$ to $\phi(x)$;
         \item For each leaf $z$ with value $y_i$ in $T_i$, assign the value $\she.\Enc(\pk,$ $y_i)$ to $\phi(z)$;
         \item For each feature name $\ell$ used in $T_i$, create the corresponding feature pseudonym $\ell^\prime \larr f(K_2, \ell)$;
        \end{itemize}
    \end{itemize}

\textbf{Proxy sends to ML Module:} $\encml$; \ \ 
\textbf{Proxy sends to client:} $\alpha$, $K_1$, $K_2$, $f$, $\sk$;

\textbf{$\query$ Phase:}\\
\textbf{Input (to client):} Query $\vect{q}$. %client computes:
\begin{itemize}[noitemsep,nolistsep, label={-}]
\item Client computes:
    \begin{itemize}[noitemsep,nolistsep]
        \item For each feature name $l$ in $\vect{q}$, compute the corresponding feature pseudonym  
              $l'\larr f(K_2, l)$;
        \item Encrypt the plaintext value: $\vect{q^\prime} \larr \OPE.\Enc(K_1, \vect{q})$;
    \end{itemize}
\item \textbf{Client sends to ML Module:} $\vect{q'}$

\item ML Module computes:
    \begin{itemize}[noitemsep,nolistsep]
          \item For each $T_i^\prime \in \encml$, evaluate $T_i^\prime$ on $\vect{q^\prime}$ to obtain value $y_i^\prime$;
          \item Homomorphically sum the values: $y^\prime \larr \SHE.\eval(+, y_1^\prime, \ldots, y_n^\prime)$, where $n$ is the number of CARTs in $\encml$;
    \end{itemize}      
    
    \item \textbf{ML Module sends to client:} $y^\prime$;
    \item Client decrypts the result: $y \larr \SHE.\Dec(\sk,$ $y^\prime$);
    \item Client interprets the result using the model hyper-parameter $\alpha$;
\end{itemize}      

}


